An actor-critic algorithm with policy gradients to solve the job shop scheduling problem using deep double recurrent agents

There is a growing interest in integrating machine learning techniques and optimization to solve challenging optimization problems. In this work, we propose a deep reinforcement learning methodology for the job shop scheduling problem (JSSP). The aim is to build up a greedy-like heuristic able to learn on some distribution of JSSP instances, different in the number of jobs and machines. The need for fast scheduling methods is well known, and it arises in many areas, from transportation to healthcare. We model the JSSP as a Markov Decision Process and then we exploit the efficacy of reinforcement learning to solve the problem. We adopt an actor-critic scheme, where the action taken by the agent is influenced by policy considerations on the state-value function. The procedures are adapted to take into account the challenging nature of JSSP, where the state and the action space change not only for every instance but also after each decision. To tackle the variability in the number of jobs and operations in the input, we modeled the agent using two incident LSTM models, a special type of deep neural network. Experiments show the algorithm reaches good solutions in a short time, proving that is possible to generate new greedy heuristics just from learning-based methodologies. Benchmarks have been generated in comparison with the commercial solver CPLEX. As expected, the model can generalize, to some extent, to larger problems or instances originated by a different distribution from the one used in training.

==> review_folder/preamble.tex <==
\usepackage[]{todonotes}
\usepackage[ruled]{algorithm2e}
\usepackage{endnotes}
\usepackage{pgfplots}
\usepackage{lscape}
\usepackage{setspace}
%\usepackage{subfigure}
\pgfplotsset{compat=newest}
\let\enotesize=\normalsize
\def\notesname{Endnotes}%
\def\makeenmark{$^{\theenmark}$}
\def\enoteformat{\rightskip0pt\leftskip0pt\parindent=1.75em
\leavevmode\llap{\theenmark.\enskip}}
\usepackage{rotating}
\usepackage{float}



\usepackage{verbatim}
 \newcommand{\cyan}[1]{\textcolor{cyan}{#1}}
 \newcommand{\red}[1]{\textcolor{red}{#1}}
 \newcommand{\blue}[1]{\textcolor{blue}{#1}}
 \newcommand{\green}[1]{\textcolor{green}{#1}}
\def\bigno{\par\bigskip\noindent} \def\pano{\par\noindent}
\def\meno{\par\medskip\noindent}
\def\eop{\vbox{\hrule\hbox{\vrule\hbox to3pt{\vbox to6pt{\vfil}\hfil}\vrule}\hrule}}

\usepackage{lscape}

\usepackage{amsmath,amsfonts,amsthm,amssymb}
\def\setR{\mathbb{R}}
\def\setN{\mathbb{N}}
\def\td{\texttt{TD} }
\def\RL{\texttt{RL} }
\def\rl{\texttt{DeepRL} }
\def\S{\mathcal{S}_t}
\def\A{\mathcal{A}_t}
\def\R{\mathcal{R}}
\def\MDP{\texttt{MDP} }
\def\PPO{\texttt{PPO} }
\def\TRPO{\texttt{TRPO} }

\newcommand{\mnote}{\textcolor{blue}}

%
%%enviroment
\usepackage{footnote}
\makesavenoteenv{tabular}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{problem}{Problem}

%\addtolength{\headsep}{0.25in}
%\addtolength{\headsep}{12pt}
%\addtolength{\topmargin}{-0.2in}

\textwidth 16 cm   %*******
\textheight 22 cm  %*******
\oddsidemargin 0 cm  %*******
\evensidemargin 0 cm

%\topmargin 0.6 cm  %*******

%\footskip 0.8 cm \rightmargin=\leftmargin
%\parindent 0cm	
%\renewcommand{\baselinestretch}{1.5}

\graphicspath{{./figures/}}

\usepackage{comment}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{adjustbox}
\usepackage{tikz}
\usepgfplotslibrary{dateplot}
\usepgfplotslibrary{groupplots}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{psfrag}
\usepackage{soul}
\usepackage{mwe}

\usepgfplotslibrary{fillbetween}

\usetikzlibrary{er,positioning, calc, shapes, arrows, chains, fit}

\definecolor{myblue}{RGB}{19,145,215}
%\definecolor{mygreen}{RGB}{65,144,40}
\definecolor{mygreen}{RGB}{80,176,50}
\definecolor{myred}{RGB}{222,36,16}

%istanze Taillard (rileggere)


%FIFO 
%MWKR
%OPT
%LPT
%SPT
%FDD/MWKR
%MOPNR
%GA (Priority rule)
%SPT+SSO
%LPT+LSO
%iterative repair (IR) method of Zweben
%shuLtle payload processing jobs


%prova solo con 50x45

%15x10
%20x15
%25x20
%30x25
%35x30
%40x35
%45x40
%50x45

%40x10
%50x20

%100 ciascuna

%riempire altro migliaio, 10 da 100, o 5
%da 35x30 fino a 50x45

%Episodi 10000?
